DebFilter: Eradicating Biases Stashed in Value

Text-to-image diffusion models, which are theoretically equivalent to score-based generative models, generate images through a multi-step denoising process guided by text embeddings extracted from pretrained vision-language models such as CLIP. However, these text embeddings inherently encode social and semantic biases -- such as those related to gender and age -- that are subsequently propagated and amplified through the guidance mechanism, along with the model's training on large-scale datasets that are imbalanced with respect to these bias-related concepts, often leading to skewed outputs in text-to-image generation. We propose DebFilter, a lightweight and training-free framework for mitigating such biases in text-to-image diffusion models. Observing that the model's error prediction at each denoising step is primarily influenced by cross-attention dynamics, we introduce a bias-correction strategy that adjusts the value components within cross-attention. Specifically, we apply a fixed offset to the slice of guidance embedding, effectively steering the semantic direction of cross-attention values toward unbiased representations. This adjustment reconfigures the score landscape to produce balanced outputs while maintaining alignment with the intended text semantics. Unlike prior approaches that rely on fine-tuning or retraining, DebFilter operates entirely at inference time, requiring no additional data or model updates. Our results demonstrate that this method effectively mitigates social biases in generated images, offering an efficient and scalable pathway toward fairer and more inclusive text-to-image generation.

==> sec/4_experiments_.tex <==
\section{Experiments}
\label{results}
We evaluated our method using SD(Stable Diffusion V2.1) as a baseline model. The denoising U-Net in SD has a depth of 3, and each encoder depth contains two transformers, with each transformer comprising both a self-attention and a cross-attention mechanism. The bottleneck consists of a single transformer, while the decoder contains three transformers. As a result, a single denoising step involves a total of 16 cross-attention operations. Our filtering process is applied based on this number of cross-attentions.

We selected three professions—\textit{CEO}, \textit{firefighter}, and \textit{driver}—to construct \textbf{DebFilter}, and exclude these from the set of professions during evaluation.

Unlike previous studies that apply debiasing uniformly across all generated images, our approach enables pre-specifying the proportion of samples to be debiased. As shown in Table~\ref{tab:occupation_all}, the Transition Scores (TS)~\ref{ts} for most occupations closely align with the target ratio of 0.5. This demonstrates that \textbf{DebFilter} not only achieves approximate gender parity but also allows for flexible and controlled adjustment of the debiasing ratio. 

\subsection{Gender Bias Mitigation}
\label{sec:exp-gender}

With the aid of WinoBias~\cite{zhao2018gender} and DALL-Eval~\cite{Cho2023DallEval}, we select a total of 87 occupations, consisting of 58 male-dominant occupations—predominantly represented by men—and 29 female-dominant occupations—mostly represented by women—for image generation. While WinoBias categorizes certain occupations as socially male- or female-dominated, we observe that the gender distribution in generated outputs is often inverted. To investigate this discrepancy, we generate images for each occupation using a neutral prompt such as ``A person who works as \([occupation]\)'' with the vanilla SD model. We then estimate gender distributions using CLIP (ViT-B/32)~\cite{radford2021learning}-based few-shot classification. Based on these results, we conduct a series of debiasing experiments under various conditions.

\subsubsection{Evaluation Metrics}
\paragraph{Bias Ratio \(\Delta_{p}\)} 
Following prior work such as TIME~\cite{orgad2023editing} and UCE~\cite{gandikota2024unified}, we calculate the proportion of generated female-presenting figures for each profession, denoted as \( F_p \in [0, 100] \), to assess gender inequality in the model's representation of professions. For each prompt, we generate 120 images and use CLIP to classify gender in the generated outputs. 

We then compute the gender bias for each profession using the normalized absolute deviation of \( F_p \) from the ideal 50\% balance, given by: \(\Delta_p = \frac{|F_p - 50|}{50}\).
To obtain an overall gender bias metric for the model, we average \( \Delta_p \) across all professions: \(\Delta = \frac{1}{|P|} \sum_{p \in P} \Delta_p\) where \( P \) is the set of all evaluated professions. A lower \( \Delta = 0 \) indicates a more balanced results and a perfectly unbiased model would yield \( \Delta = 0 \).
\begin{table*}[ht]
\centering
\vspace{0.5em}
\small
\begin{minipage}[t]{0.31\textwidth}
    \centering
    (a) Male-dominant occupations
    % \label{tab:occupation_male}
    \vspace{0.5em}
    \begin{tabular}{@{}lccc@{}}
        \toprule
        \textbf{Occupation} & \(\Delta_{org}\downarrow\) & \(\Delta_{deb}\downarrow\) & TS \\
        \midrule
        scientist    & 0.783 & 0.067 & 0.40 \\
        engineer     & 0.883 & 0.050 & 0.49 \\
        doctor       & 0.617 & 0.250 & 0.53 \\
        sheriff      & 0.492 & 0.017 & 0.46 \\
        journalist   & 0.783 & 0.017 & 0.43 \\
        electrician  & 0.983 & 0.033 & 0.48 \\
        plumber      & 0.983 & 0.033 & 0.48 \\
        mechanic     & 1.000 & 0.050 & 0.48 \\
        cook         & 0.817 & 0.117 & 0.51 \\
        manager      & 0.683 & 0.017 & 0.42 \\
        \bottomrule
    \end{tabular}
\end{minipage}
\hspace{0.02\textwidth}
\begin{minipage}[t]{0.31\textwidth}
    \centering
    (b) Female-dominant occupations
    % \label{tab:occupation_female}
    \vspace{0.5em}
    \begin{tabular}{@{}lccc@{}}
        \toprule
        \textbf{Occupation} & \(\Delta_{org}\downarrow\) & \(\Delta_{deb}\downarrow\) & TS \\
        \midrule
        nurse             & 0.950 & 0.050 & 0.45 \\
        dentist           & 0.317 & 0.017 & 0.49 \\
        caretaker         & 0.467 & 0.200 & 0.33 \\
        hairdresser       & 0.317 & 0.417 & 0.38 \\
        translator        & 0.883 & 0.067 & 0.28 \\
        civil servant     & 0.183 & 0.117 & 0.42 \\
        teacher           & 0.383 & 0.233 & 0.37 \\
        police officer    & 0.417 & 0.133 & 0.38 \\
        personal assistant& 0.817 & 0.017 & 0.41 \\
        makeup artist     & 1.000 & 0.383 & 0.30 \\
        \bottomrule
    \end{tabular}
\end{minipage}
\hspace{0.02\textwidth}
\begin{minipage}[t]{0.31\textwidth}
    \centering
    (c) CLIPScore comparison
    \vspace{0.5em}
    \begin{tabular}{@{}lcc@{}}
        \toprule
        \textbf{Occupation} & \textbf{Vanilla} & \textbf{DebFilter} \\
        \midrule
        Teacher     & 26.30 & \textbf{26.51} \\
        Librarian   & \textbf{29.10} & 28.85 \\
        Lawyer      & 27.53 & \textbf{28.17} \\
        Doctor      & \textbf{29.09} & 28.90 \\
        Sheriff     & \textbf{30.63} & 30.43 \\
        Executive   & 26.68 & \textbf{27.24} \\
        \midrule
        Mean        & 27.08 & \textbf{27.91} \\
        \bottomrule
    \end{tabular}
    % \label{tab:clip-scores}
\end{minipage}
\caption{Debiasing performance across occupations. (a) Male-dominant and (b) female-dominant occupations show substantial reductions in occupational bias after applying \textit{DebFilter}. (c) CLIPScore comparison indicates that DebFilter achieves comparable or improved alignment quality relative to the vanilla model.}
\label{tab:occupation_all}
\end{table*}

% \begin{table*}[ht]
% \centering
% \caption{Comparison of old and new \(\Delta\) for selected occupations}
% % \vspace{0.5em}
% {\small % Reduce text size for both tables
% \begin{minipage}[t]{0.3\textwidth}
% \centering
% \textbf{(a) Male-dominant occupations}
% \vspace{0.5em}
% \begin{tabular}{@{}l@{\hskip 3pt}c@{\hskip 3pt}c@{\hskip 3pt}c@{}}
% \toprule
% \textbf{Occupation} & \(\Delta_{org}(\downarrow)\) & \(\Delta_{deb}(\downarrow)\) & TS \\
% \midrule
% scientist    & 0.783 & 0.067 & 0.40 \\
% engineer     & 0.883 & 0.050 & 0.49 \\
% doctor       & 0.617 & 0.250 & 0.53 \\
% sheriff      & 0.492 & 0.017 & 0.46 \\
% journalist   & 0.783 & 0.017 & 0.43 \\
% electrician  & 0.983 & 0.033 & 0.48 \\
% plumber      & 0.983 & 0.033 & 0.48 \\
% mechanic     & 1.000 & 0.050 & 0.48 \\
% cook         & 0.817 & 0.117 & 0.51 \\
% manager      & 0.683 & 0.017 & 0.42 \\
% \bottomrule
% \end{tabular}
% \label{tab:occupation_male}
% \end{minipage}
% \hspace{0.02\textwidth}
% \begin{minipage}[t]{0.3\textwidth}
% \centering
% \textbf{(b) Female-dominant occupations}
% \vspace{0.5em}
% \begin{tabular}{@{}l@{\hskip 3pt}c@{\hskip 3pt}c@{\hskip 3pt}c@{}}
% \toprule
% \textbf{Occupation} & \(\Delta_{org}(\downarrow)\) & \(\Delta_{deb}(\downarrow)\) & TS \\
% \midrule
% nurse             & 0.950 & 0.050 & 0.45 \\
% dentist           & 0.317 & 0.017 & 0.49 \\
% caretaker         & 0.467 & 0.200 & 0.33 \\
% hairdresser       & 0.317 & 0.417 & 0.38 \\
% translator        & 0.883 & 0.067 & 0.28 \\
% civil servant     & 0.183 & 0.117 & 0.42 \\
% teacher           & 0.383 & 0.233 & 0.37 \\
% police officer    & 0.417 & 0.133 & 0.38 \\
% personal assistant& 0.817 & 0.017 & 0.41 \\
% makeup artist     & 1.000 & 0.383 & 0.30 \\
% \bottomrule
% \end{tabular}
% \label{tab:occupation_female}
% \end{minipage}
% } % End small
% \label{tab:occupation_comparison}
% \end{table*}

Since the gender distribution for each prompt is unknown and may vary depending on the random seed, we uniformly set \(p = 0.5\) for all experiments. Table~\ref{tab:occupation_all}(a) demonstrates that \textbf{DebFilter} with \(p=0.5\) effectively mitigates gender bias across a range of occupations. \(\Delta_{\text{org}}\) and \(\Delta_{\text{debiased}}\) refer to the \(\Delta\) values obtained from vanilla SD and after applying DebFilter with \(p = 0.5\), respectively. Although the debiasing ratio is set to 0.5, the resulting \( \Delta \) may remain greater than zero, as the initial \( F_{p} \) values from the vanilla generation are not uniformly skewed toward 100\% or 0\%, but vary across occupations. However, for most occupations, the TS remains close to 0.5, indicating that \textbf{DebFilter} successfully enforces the target debiasing ratio in practice. 

With analyzing the gender distribution from the vanilla generation and then adjusting the debiasing ratio of \textbf{DebFilter} accordingly, it is possible to generate outputs with gender proportions that result in a \( \Delta \) value closer to zero across occupations.

Compared to TIME and UCE in Table~\ref{tab:delta-comparison}, \textbf{DebFilter} outperformed in randomly selected professions in UCE. Here we used SDXL~\cite{podell2023sdxl} as a baseline model in order to compare \(\Delta\) with recent studies.
\begin{figure}[tbp]
    \centering
    \includegraphics[width=\linewidth]{fig/delta-compare.pdf}
    \caption{Comparison of bias reduction(\(\Delta\)) across professions for different debiasing models. Lower \(\Delta\) implies more balanced results.}
    \label{tab:delta-comparison}
\end{figure}
% \begin{table*}[ht]
% \centering
% \small
% \caption{Comparison of bias reduction(\(\Delta\)) across professions for different debiasing models}
% \begin{tabular}{@{}lcccc@{}}
% \toprule
% \textbf{Profession} & \textbf{SD}\((\Delta\downarrow)\) & \textbf{TIME}\((\Delta\downarrow)\) & \textbf{UCE}\((\Delta\downarrow)\) & \textbf{DebFilter}\((\Delta\downarrow)\) \\
% \midrule
% \textit{Librarian} & $0.88 \pm 0.02$ & $0.25 \pm 0.05$ & $0.07 \pm 0.07$ & $\mathbf{0.06 \pm 0.01}$ \\
% \textit{Teacher} & $0.38 \pm 0.04$ & $0.34 \pm 0.06$ & $0.06 \pm 0.02$ & $\mathbf{0.02 \pm 0.03}$ \\
% \textit{Sheriff} & $0.90 \pm 0.01$ & $0.22 \pm 0.05$ & $0.10 \pm 0.03$ & $\mathbf{0.01 \pm 0.01}$ \\
% \textit{Analyst} & $0.58 \pm 0.10$ & $0.52 \pm 0.03$ & $0.20 \pm 0.07$ & $\mathbf{0.15 \pm 0.08}$ \\
% \textit{Doctor} & $0.62 \pm 0.08$ & $0.58 \pm 0.03$ & $0.20 \pm 0.07$ & $\mathbf{0.13 \pm 0.03}$ \\
% \bottomrule
% \end{tabular}
% \label{tab:delta-comparison}
% \end{table*}

To examine the applicability of our approach to various scenarios, we conducted an experiment by applying the \( \Delta{G} \) obtained from the male-dominant examples with the opposite sign. Table~\ref{tab:occupation_all}(b) illustrates that the \(\Delta G\) obtained from male-to-female debiasing can produce a comparable effect when applied in the reverse direction (i.e., as a female-to-male filter by simply inverting the direction). This demonstrates that DebFilter can compute in the opposite direction simply by changing the sign similar to vector operations. Consequently, there is no need to separately compute and store \( \Delta G \) for modifications from female to male.

\paragraph{Transition Score}
\label{ts}
Similar to Recall from FACET~\cite{gustafson2023facet},  we define the proportion of these altered outputs as the \textit{Transition Score}, which quantifies the extent of adjustment during debiasing.
\begin{equation}
\text{Transition Score} = 
\begin{cases}
\frac{\#(\text{male} \rightarrow \text{female})}{\#(\text{original male})}, & \text{reducing male bias}, \\
\frac{\#(\text{female} \rightarrow \text{male})}{\#(\text{original female})}, & \text{reducing female bias}.
\end{cases}
\notag
\end{equation}

\paragraph{\textit{Skew}}SFID~\cite{jung2024unified} measured a fairness of generative models to produce an equal number of images for each gender across all occupations. Accordingly, the bias metric quantifies the degree of \textit{Skew} in the gender distribution of the generated outputs:
{\small
\[
\text{\textit{Skew}} = \frac{1}{|P|} \sum_{p \in P} \frac{\max(N_{p,m}, N_{p,f})}{C}
\]
}
where \( N_{p,m} \) and \( N_{p,f} \) denote the number of detected male and female images, respectively, for occupation \( p \), and \(C\) is the number of image generations per prompt. In an ideal case with no bias, the \textit{Skew} value would be 50.

\begin{table}[tb]
\centering
\footnotesize
\vspace{4pt}
% \setlength{\tabcolsep}{3.5pt} % tighter column spacing
\begin{tabular}{lrrrrrr}
\toprule
\textbf{Method} & Base & DeAR & Cl-clip & P-Deb & SFID & DebFilter \\
\midrule
\textit{Skew} & 83.25 & 99.88 & 82.05 & 82.77 & 81.57 & \textbf{62.10} \\
\bottomrule
\end{tabular}
\caption{Neutral prompt score (↓ lower is better). The methods include: Baseline, Debiasing via Regularization (DeAR), 
CLIP-clip (C-clip), Prompt-Debias (P-Deb), Selective Feature Injection with Disentanglement using a hard constraint (SFID), and DebFilter (DebF)}
\label{tab:skew}
\end{table}

Table~\ref{tab:skew} reports the \textit{Skew} values across various debiasing methods, measuring the degree of gender imbalance in the generated images for a set of occupation prompts. Lower values indicate fairer gender distributions. While most methods show moderate improvements or even regressions compared to the baseline, \textbf{DebFilter} achieves the lowest \textit{Skew} score of 62.1, demonstrating its effectiveness in mitigating gender bias across prompts.

Figure \ref{fig:m2f} shows that DebFilter modifies only gender-specific details while keeping the overall image layout intact. Averaging $\Delta G_{debias}^{gender}$ across three random jobs, we found that male-to-female changes mainly involve clothing, hairstyle, makeup, skin texture, and arm thickness. Reversing $\Delta G$ transforms female to male with similar changes, mirroring the male-to-female direction.
\begin{figure}[htbp]
    \centering
    \begin{subfigure}{0.9\linewidth}
        \includegraphics[width=\linewidth]{fig/gender-bias.pdf}
        \caption{Gender bias mitigation}
        \label{fig:m2f}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.9\linewidth}
        \includegraphics[width=\linewidth]{fig/age-bias.pdf}
        \caption{Age bias mitigation}
        \label{fig:e2y}
    \end{subfigure}
    \caption{Examples where the gender-bias (left) and age-bias (right) are mitigated using \textit{DebFilter}.}
\end{figure}

\paragraph{CLIPScore} 
To further analyze the quality of debiased images, we calculate the CLIPScore for each image under different prompting conditions. Specifically, we use female-explicit prompts (e.g., ``A female sheriff'') when assessing CLIPScore for filtered images that have been transformed from male to female or vice versa.

% \begin{table}[htbp]
%     \small
%     \centering
%     \begin{tabular}{lcc}
%     \toprule
%     \textbf{Occupation} & \textbf{Vanilla} & \textbf{DebFilter} \\
%     \midrule
%     Teacher     & 26.3  & \textbf{26.51} \\
%     Librarian   & \textbf{29.1}  & 28.85 \\
%     Lawyer      & 27.53 & \textbf{28.17} \\
%     Doctor      & \textbf{29.09} & 28.9 \\
%     Sheriff     & \textbf{30.63} & 30.43 \\
%     Executive   & 26.68 & \textbf{27.24} \\
%     \midrule
%     Mean        & 27.08 & \textbf{27.91} \\
%     \bottomrule
%     \end{tabular}
%     \vspace{4pt}
%     \caption{CLIPScores Comparison Between Vanilla Method and DebFilter}
%     \label{tab:clip-scores}
% \end{table}

\textbf{DebFilter} is capable of effectively addressing the target bias without compromising the original semantic content or meaning of the generated outputs. As can be seen from Table~\ref{tab:occupation_all}(c), \textbf{DebFilter} achieves comparable or even higher scores compared to the CLIPScores obtained using the vanilla model, demonstrating that it produces results that more faithfully align with the given prompt.

\subsection{Age Bias Mitigation}
\label{sec:exp-age}
Broadly, age in bias mitigation area is classified into three categories: young (0–30), middle-aged (31–60), and elderly (60+). Certain words representing professions or individuals tend to be associated with either young or elderly age groups. Similar to Gender Bias Mitigation, we choose 14 words that refer to a person performing a specific action for evaluation(e.g., clock-maker). 

The samples in the top row of Figure \ref{fig:e2y} demonstrate that prompts containing certain professions such as ``clockmaker" or ``philosopher" exhibit a bias toward generating only older individuals while ``barista'' or ``student'' shows the opposite.
To make \textbf{DebFilter} for age, \( \Delta{G} \) is computed with target prompt that `\textit{young}' is inserted in front of the subject of source prompt(e.g., the target prompt of ``A blacksmith forging metal in an old workshop" becomes ``A \textit{young} blacksmith forging metal in an old workshop").

In the same manner as described in debiasing female-dominant cases, the \textbf{DebFilter} for elderly-to-young transformation was stored and applied in the reverse direction. Figure~\ref{fig:e2y} shows that not only the appearance of a person such as hair style or wrinkles in skin is changed, style of the outfit also naturally changed compared to original samples. Though the action or social role is awkward with the age, \textbf{DebFilter} translates the semantic information naturally within the unchanged backgrounds.

\subsection{Multi-Object}
\label{sec:exp-multi}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.85\linewidth]{fig/multis.pdf}
    \caption{Gender-reversed examples of ``A doctor and a nurse", ``A lawyer and a client" and ``A scientist with an assistant".}
    \label{fig:multi-object}
\end{figure}
Previous studies have focused on mitigating bias solely in the context of single objects. While TIME\cite{orgad2023editing} find it hard to control multiple professions at the same time, we further demonstrate that our proposed method can be applied to multi-object scenarios as well. While the \textit{Value} corresponding to male-dominant object (e.g., `doctor') is filtered, the \textit{Value} corresponding to female-dominant object(e.g., `nurse') is refined in the opposite direction at the same time.

The examples in the lower row of Figure~\ref{fig:multi-object} clearly show that the original image of a male (in the upper row) is filtered to appear as a female, and vice versa for the original image of a female. Notably, these transformations preserve the overall layout and background of the images. Additional examples of applying \textbf{DebFilter} to various object combinations can be found in the Supplementary Materials.
